Learning about an exponential amount of conditional distributions

We introduce the Neural Conditioner (NC), a self-supervised machine able to learn about all the conditional distributions of a random vector $X$. The NC is a function $NC(x \cdot a, a, r)$ that leverages adversarial training to match each conditional distribution $P(X_r|X_a=x_a)$. After training, the NC generalizes to sample from conditional distributions never seen, including the joint distribution. The NC is also able to auto-encode examples, providing data representations useful for downstream classification tasks. In sum, the NC integrates different self-supervised tasks (each being the estimation of a conditional distribution) and levels of supervision (partially observed data) seamlessly into a single learning experience.

==> experiments.tex <==
\section{Experiments}





\subsection{Three-dimensional Gaussians}

We consider data $(x_1, \ldots, x_n)$ containing examples
\begin{equation*}
    x_i \sim \mathcal{N}\left(
        (2, 4, 6),
        \begin{bmatrix} 1 & \rho & \rho^2 \\ \rho & 1 & 0 \\ \rho^2 & 0 & 1 \end{bmatrix}
        \right).
\end{equation*}
Using random masks $(a, r)$ following a Bernoulli distribution, we are interested in designing an NPM to estimate all the Gaussian conditional expectations $p(x_r | x_a)$.
%
Since we have a closed-form expression for the true Gaussian conditional expectations governing the data, this experiment serves as a sanity check on our approach.

In this experiment, our machine $\hat{x} = M(x_a, a, r, z)$ is an MLP with a single hidden layer of $512$ neurons and ReLU nonlinearities, and $z \sim \mathcal{N}(0, I)$.
%
The contrast function $T$ is a network of the same architecture, trained to distinguish between real samples $(x_a, x_r, a, r)$ and fake samples $(x_a, \hat{x}, a, r)$.
%
Note how we do not mask $\hat{x}$ a posteriori with $r$.
\begin{itemize}
    \item Quantitative results: Table~\ref{table:mmd} shows the Maximum Mean Discrepancy (MMD) and Energy Distance (ED) statistics between the estimated and true conditional distributions, showing a reasonable degree of accuracy.
    %
    \item Qualitative results: Figure~\ref{fig:densities} visualizes two examples of estimated versus true conditional distributions.
    %
    \item We observe different behavior for overlaping/non-overlaping $(a, r)$!
    %
    \item Negative result: masking generations $\hat{x}$ with $r$ a posteriori does not work!
\end{itemize}

\begin{table}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{llrrrrrrrrrrrrrrrr}
        \toprule
                &           & \multicolumn{8}{l}{Energy statistic} & \multicolumn{8}{l}{MMD Statistic} \\
                &           &  count &  mean &   std &   min &  25\% &  50\% &  75\% &   max &  count &  mean &   std &   min &  25\% &  50\% &  75\% &   max \\
              $A$ &       $R$ &        &       &       &       &       &       &       &       &        &       &       &       &       &       &       &       \\
        \midrule
        (1, 0, 0) & (0, 0, 1) &   20.0 &  0.04 &  0.04 &  0.00 &  0.00 &  0.02 &  0.06 &  0.14 &   20.0 &  0.03 &  0.03 &  0.00 &  0.00 &  0.01 &  0.05 &  0.11 \\
                  & (0, 1, 0) &   20.0 &  0.07 &  0.08 &  0.01 &  0.02 &  0.03 &  0.10 &  0.29 &   20.0 &  0.06 &  0.06 &  0.01 &  0.02 &  0.03 &  0.08 &  0.22 \\
                  & (0, 1, 1) &   20.0 &  0.05 &  0.06 &  0.01 &  0.02 &  0.02 &  0.04 &  0.22 &   20.0 &  0.03 &  0.03 &  0.01 &  0.01 &  0.02 &  0.03 &  0.12 \\
        (0, 1, 0) & (0, 0, 1) &   20.0 &  0.09 &  0.10 &  0.00 &  0.02 &  0.06 &  0.14 &  0.37 &   20.0 &  0.07 &  0.07 &  0.00 &  0.01 &  0.05 &  0.10 &  0.24 \\
                  & (1, 0, 0) &   20.0 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.01 &  0.02 &   20.0 &  0.01 &  0.00 &  0.00 &  0.00 &  0.01 &  0.01 &  0.02 \\
                  & (1, 0, 1) &   20.0 &  0.01 &  0.01 &  0.00 &  0.01 &  0.01 &  0.01 &  0.04 &   20.0 &  0.01 &  0.01 &  0.00 &  0.00 &  0.01 &  0.01 &  0.03 \\
        (0, 0, 1) & (0, 1, 0) &   20.0 &  0.05 &  0.05 &  0.00 &  0.01 &  0.02 &  0.06 &  0.20 &   20.0 &  0.04 &  0.04 &  0.01 &  0.01 &  0.02 &  0.05 &  0.15 \\
                  & (1, 0, 0) &   20.0 &  0.01 &  0.00 &  0.00 &  0.01 &  0.01 &  0.01 &  0.02 &   20.0 &  0.01 &  0.01 &  0.01 &  0.01 &  0.01 &  0.01 &  0.03 \\
                  & (1, 1, 0) &   20.0 &  0.02 &  0.02 &  0.00 &  0.01 &  0.01 &  0.02 &  0.06 &   20.0 &  0.01 &  0.01 &  0.00 &  0.00 &  0.01 &  0.01 &  0.03 \\
        (1, 0, 1) & (0, 1, 0) &  400.0 &  0.38 &  0.82 &  0.00 &  0.01 &  0.02 &  0.10 &  3.91 &  400.0 &  0.23 &  0.47 &  0.00 &  0.01 &  0.02 &  0.08 &  2.05 \\
        (1, 1, 0) & (0, 0, 1) &  400.0 &  0.16 &  0.35 &  0.00 &  0.00 &  0.01 &  0.06 &  1.89 &  400.0 &  0.11 &  0.23 &  0.00 &  0.00 &  0.01 &  0.05 &  1.20 \\
        (0, 1, 1) & (1, 0, 0) &  400.0 &  0.02 &  0.05 &  0.00 &  0.00 &  0.00 &  0.02 &  0.28 &  400.0 &  0.02 &  0.04 & -0.00 &  0.00 &  0.01 &  0.01 &  0.20 \\
        \bottomrule
        \end{tabular}
    }
    \caption{%
        MMD and Energy distances estimated conditional distributions and ground truth.
        %
        When $\|a\|_1 = 1$, we sample from all conditioning values in a 20-dimensional grid $[\mu - 3 \sigma, \mu + 3 \sigma]$.
        %
        When $\|a\|_1 = 2$, we sample from the cross-product of the grids of the available marginals.
    }
    \label{table:mmd}
\end{table}


\begin{figure}[t]
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=0.99\linewidth]{./figures/cond_density_gaussian_100_011_184.png}
    \end{minipage}
    \hfill
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=0.99\linewidth]{./figures/cond_density_gaussian_100_001_244.png}
    \end{minipage}
    \caption{Samples of estimated versus true conditional densities.}
    \label{fig:densities}
\end{figure}

\subsection{SVHN}

In this experiment, we use the Street View House Numbers (SVHN) dataset to apply NPM to natural images.
%
Here, the masks $(a, r)$ are random rectangles occupying a size from $10\%$ to $50\%$ of the total image.

In this experiment, the NPM takes the form:
\begin{equation*}
    M(x_a, a, r) = \text{Decoder}(\text{Encoder}(x_a, a, r)).
\end{equation*}
%
In the spirit of VAEs, the Encoder i) is a 4-layer CNN that ii) outputs a latent code $z = (\mu, \sigma) \in \mathbb{R}^{128}$, and iii) sends a sample from $\mathcal{N}(\mu, \text{diag}(\sigma^2))$ to the Decoder.
%
The Decoder is also a 4-layer CNN producing the generation $\hat{x}$.
%
The contrast function $T$ is a 4-layer CNN trained to distinguish between real samples $(x_a, x_r, a, r)$ and fake samples $(x_a, \hat{x}, a, r)$.
%
Again, note that we do not mask $\hat{x}$ a posteriori with $r$.
%
We regularize the contrast function with:
\begin{align*}
    \mathbb{E}_x \left[\|\nabla_x D(x_a, x_r, a, r)\|\right] + \mathbb{E}_z \left[\|\nabla_{\hat{x}} D(x_a, \hat{x}, a, r)\| \right].
\end{align*}
%
The discriminator is updated 5 times for every generator update.
%
We use partial convolutions \citep{liu2018image} in the discriminator and generator.
%
We provide a max-pooled version of the requested mask $r$ to the input of each convolutional layer of the Decoder.
%
In our experiments, we observe:
\begin{itemize}
    \item Different stochastic evaluations of the Encoder lead to different generations. %(Figure~\ref{fig:svhn_qualitative}).
    \item If with probability $p$ we give the empty mask $a = 0$ and the full mask $r = 1$ (c.f. GANs), the generator is able to generate entire new samples. %(Figure~\ref{fig:svhn_flip}).
    \item We obtain the same effect (ability to generate full samples) if we
      regularize the latent code $z$ with by minimizing the Kullblack-Leibler
      divergence between the approximate posterior and standard gaussian (Figure~\ref{fig:svhn_zreg}).
    \item The previous point is evidence about the ability of NPMs to generalize to masks not seen during training.
\end{itemize}

\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{figures/svhn_projections_no_R.png}
  \caption{%
    SVHN projections. The decoder is not explicitly provided with $r$.
    %
    Columns are: $x_a$, $x_r$, $\hat{x}_r$, $\hat{x}$, $x_a + \hat{x}_r$, $x$.}
\end{figure}


\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{figures/svhn_projections_with_R.png}
  \caption{%
      SVHN projections. The decoder is explicitly provided with $r$ at each layer
      %
      Columns are: $x_a$, $x_r$, $\hat{x}_r$, $\hat{x}$, $x_a + \hat{x}_r$, $x$.}
\end{figure}

\begin{figure}
  \label{fig:svhn_zreg}
  \begin{minipage}{0.4\textwidth}
    \centering
    (a) No Latent space regularization
    \includegraphics[width=0.99\linewidth]{./figures/svhn_with_R_samples_from_x.png}
  \end{minipage}
  \hfill
  \begin{minipage}{0.4\textwidth}
    \centering
    (b) Variational bottleneck with coefficient of $1e-3$
    \includegraphics[width=0.99\linewidth]{./figures/svhn_with_r_kl_001_samples_from_x.png}
  \end{minipage}
  \caption{Model samples with and without bottleneck in the latent space.}
\end{figure}


==> future_work.tex <==
\section{Future work}

\paragraph{What is the best way to provide $(x_a, x_r, a, r)$ to the discrminator?} 
%
We currently concatenate these variables as channels.
%
However, there is literature\citep{miyato2018cgans} exploring different conditional discriminator architectures with large differences in performance. 
%
These differences also seem to play a role in NPMs.
%
One alternative is to concatenate the images $(x_a, x_r)$ side to side, and append as channels the corresponding masks $(a, r)$.

\paragraph{What is the best way to condition the discriminator on masks?}
%
Should the discriminator access $(a, r)$ only at the input layer? Or at multiple levels of representation?

\paragraph{Should the discriminator have simultaneous access to both $x_a$ and $x_r$?}
%
One alternative is to return the inner product between the separate feature vectors $\phi(x_a, a)$ and $\phi(x_r, r)$.

\paragraph{What should the generator bottleneck depend on?}
%
Some options include $(x_a, a)$, $(x_a, a, r)$, and $(x_a, x_r)$.

\paragraph{What should the generator decoder have access to?} 
%
Providing $x_a$ would allow the decoder to copy available pixels directly.
%
Providing $r$ would allow the decoder to estimate the support of $x_r$ more easily.

\paragraph{How to choose the best masking distribution?}
%
We have observed that the sparsity implied by the randomly masked inputs significantly hampers training.
%
Do the neuronal activations show to much variance for different random masks?

\paragraph{How to mask the generations?}
%
We observed that the norm of the gradient of both discriminator and generator grow during, while the conditional samples of the generator increase in quality. 
%
However, if the output of the generator is masked a posteriori with $r$, the norm of these gradients behaves as expected, decreasing during training.
%
However, in this case the generator fails to learn the conditional distributions.


==> related_work.tex <==
\section{Related work}

The architecture of NPMs resembles an autoencoder \citep{hinton2006reducing}, and more specifically a denoising autoencoder \citep{vincent2010stacked}.
%
One of the earliest and most successful implementations of self-supervised learning is the one employed to learn word-embeddings \citep{mikolov2013distributed}.
%
Self-supervised learning problems for image data include in-painting \citep{pathak2016context}, colorization \citep{zhang2016colorful}, clustering \citep{caron2018deep}, de-rotation \citep{gidaris2018unsupervised}, or patch reordering \citep{doersch2015unsupervised, noroozi2016unsupervised}.
%
Unsupervised video is also useful to learn image features.
%
One common self-supervised learning strategy on videos is to enforce similar feature representations for nearby frames \citep{mobahi2009deep, goroshin2015unsupervised, wang2015unsupervised}, or predicting ambient sound statistics from video frames \citep{owens2016ambient}.
%
One piece of literature considered the problem of learning multiple self-supervised tasks using one network \citep{doersch2017multi}.
%
The framework of self-supervised learning has been applied successfully outside supervised learning, for instance, in reinforcement learning \citep{pathak2017curiosity}.

